Application-aware Congestion Mitigation for High-Performance Computing Systems

High-performance computing (HPC) systems frequently experience congestion leading to significant application performance variation. However, the impact of congestion on application runtime differs from application to application depending on their network characteristics (such as bandwidth and latency requirements). We leverage this insight to develop Netscope, an automated ML-driven framework that considers those network characteristics to dynamically mitigate congestion. We evaluate Netscope on four Cray Aries systems, including a production supercomputer on real scientific applications. Netscope has a lower training cost and accurately estimates the impact of congestion on application runtime with a correlation between 0.7and 0.9 for common scientific applications. Moreover, we find that Netscope reduces tail runtime variability by up to 14.9 times while improving median system utility by 12%.

==> 0001-motivation_alt.tex <==
\section{Motivation}
\label{s:motivation}
Applications running in HPC systems ~\cite{nersc_workload} have diverse communication characteristics in terms  of varying message sizes, interplay between communication primitives, and application logic. As a result, applications exhibit different sensitivity to delays (e.g., due to contention for network bandwidth) in network communications. In this context, we distinguish two broad classes of application: 
\emph{Delay sensitive} applications\footnote{We provide a definition and quantification of delay sensitivity in~\cref{s:framework}.} that rely on low link buffer occupancy to achieve minimal network latency and low application runtime.
Examples include  MILC~\cite{milc} and Quantum Espresso~\cite{quantum_benchmarking,coral_2}.
\emph{Bandwidth intensive} applications rely on large message sizes and collective communication primitives~\cite{pjevsivac2007performance} that tend to exhaust all available network bandwidth.
Examples include spectral codes~\cite{doi:10.1146/annurev.fluid.30.1.539} that use all-to-all traffic patterns.
GPCNeT~\cite{chunduri2019gpcnet} is a benchmark that mimics such bandwidth intensive behavior (i.e., all-to-all and N-to-1) in HPC applications. 
Note that there exists an entire spectrum of applications that can be found at varying levels of delay sensitivity and bandwidth intensity. 

These applications contend with each other for limited network resources, and failure to multiplex network resources efficiently leads to runtime variability and suboptimal workload completion times. \RED{Our goal is to increase the efficiency and performance of HPC systems. The following 3 insights provide key elements for achieving our goal. (or some such) This section is supposed to be Motivation so should be explicit somewhere about why the material contained in this section is in this section.}

  
 
\begin{figure*}[ht]
	\begin{subfigure}[c]{0.325\textwidth}
    \includegraphics{resources/motivation/network_counters.pdf}
    \caption{Variable impact of congestion on MILC and GPCNeT runtime as captured by low and high network stall counters}
    \label{fig:network_counters}
    \end{subfigure}
    \begin{subfigure}[c]{0.325\textwidth}
   \includegraphics{resources/motivation/workload_composition.pdf}
    \caption{Workload composition on three generations of NERSC production supercomputers}
    \label{fig:workload_composition}
    \end{subfigure}
	\begin{subfigure}[c]{0.325\textwidth}
    \includegraphics{resources/motivation/traffic_variation.pdf}
    \caption{Variation in cumulative per node traffic injection across the application's lifespan for MILC and LAMMPS}
    \label{fig:traffic_variation}
    \end{subfigure}
\caption{Characterizing high-performance computing workloads}
\end{figure*}

Development of a data-driven approach that uses application communication characteristics to guide application-aware congestion mitigation was motivated by two insights discussed below. 

\textbf{Insight 1: Application runtime variability can be reduced by augmenting the CC mechanism with awareness of application delay sensitivity.}
Congestion signals used in rate control mechanisms such as Explicit Congestion Notification~\cite{ramakrishnan2001addition}, Quantized-Congestion Notification~\cite{pan2007qcn}, and network delay~\cite{mittal2015timely,kumar2020swift} do not address the source of congestion directly.
Consequently, during the operation of the CC mechanism, the non-congestion-contributing applications are penalized along with the culprit that is responsible for the congestion. 
Moreover, if the application that is not responsible for congestion is also delay sensitive, \RED{its} performance degradation due to congestion mitigation can be severe. 
Because of inaccuracy in generating congestion signals, use of CC has been disabled on Sierra and Summit~\cite{chunduri2019gpcnet} systems (ranked second and third among the ``TOP500'' supercomputers~\cite{top_500}).


\begin{table}[ht]
\spacefigure
\centering
{%
\begin{tabular}{@{}cccc@{}}
\toprule
& Cray   & DCQCN  & \begin{tabular}[c]{@{}c@{}}Application-Aware\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}c@{}}MILC (Baseline: 26 sec)\end{tabular}   & 115\% & 58\% & 7\% \\
\begin{tabular}[c]{@{}c@{}}GPCNeT (Baseline: 75 sec)\end{tabular} & 0\% & 2.7\% & 2.7\% \\
\bottomrule
\end{tabular}%
}
\caption{Measured percentage increase in application runtime with respect to baseline for three CC mechanisms.} 
\label{tab:congestion_comparison}
\spacefigure
\end{table}


\textbf{Insight 2: Network performance counter\footnote{Network performance counters such as link stall times and traffic can be collected at switches via vendor-provided mechanisms.} telemetry data can be used to estimate application delay sensitivity.}
Network performance counters are widely collected on production systems~\cite{agelastos2014lightweight} and can be used to characterize network  behaviour. \cref{fig:network_counters} shows the runtime for MILC and GPCNeT under low (0.25\% percent time stalled\footnote{Percent Time Stalled is a proxy for measuring congestion in credit-based flow control networks that we describe in \cref{s:model}}) and high  (7.5\% percent time stalled) congestion, as measured from network stall counters. 
As expected, \cref{fig:network_counters} indicates that runtime impact of congestion varies across applications.
For instance, MILC has a 60\% increase in runtime, while GPCNeT's runtime marginally increases by 2.6\% for the same difference in measured congestion. 
We can leverage the knowledge on application behavior variability  (as measured from network performance counters) to enable estimation of applications delay sensitivity.


\end{enumerate*}







==> 0003-description.tex <==
\section{Background}
\label{s:description}













 



==> 0007-discussion.tex <==
\section{Discussion}
\label{s:discussion}



==> 0010-acknowledgements.tex <==
\section{Acknowledgements}
\label{s:acknowledgements}

This research used resources of the National Energy Research Scientific Computing Center (NERSC), a U.S. Department of Energy Office of Science User Facility operated under Contract No. DE-AC02-05CH11231. We would also like to thank Larry Kaplan and Eric Roman for fruitful discussions and suggestions.


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX
